Synchronous Pre-biasing of Triboelectric Nanogenerator for Enhanced Energy Extraction

Triboelectric Nanogenerator (TENG) is a class of ambient mechanical energy harvesters used to augment the battery life of electronic devices such as sensors in implantables, wearables, and Internet of Things (IoT) applications. In this work, the fundamentals of pre-biasing (pre-charging) the TENG at the start of the operation cycle to enhance the per-cycle extracted energy is presented. The energy gain is mathematically formulated, and the optimum pre-biasing voltage (equivalently charge) is derived by analyzing the energy exchange between the mechanical and the electrical domain over a periodic cycle. Further, a novel Energy Extraction Circuit (EEC) termed as "Pre-biased Synchronous Charge Extraction (pSCE)" is introduced to 1) Realize synchronous pre-biasing of TENG using the load battery itself and 2) Achieve enhanced energy extraction from TENG. Energy output per-cycle is derived analytically for the pSCE circuit and compared to the state of the art Synchronous Charge Extraction (SCE) circuit. The experimental implementation is performed for the proposed pSCE circuit that shows a 6.65 fold gain over the Full Wave Rectifier (standard EEC) and 1.45 over the SCE circuit for a 5V battery load.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
